Unearthing Skill-Level Insights for Understanding Trade-Offs of Foundation Models

With models getting stronger, evaluations have grown more complex, testing multiple skills in one benchmark and even in the same instance at once. However, skill-wise performance is obscured when inspecting aggregate accuracy, under-utilizing the rich signal modern benchmarks contain. We propose an automatic approach to recover the underlying skills relevant for any evaluation instance, by way of inspecting model-generated rationales. After validating the relevance of rationale-parsed skills and inferring skills for $46$k instances over $12$ benchmarks, we observe many skills to be common across benchmarks, resulting in the curation of hundreds of skill-slices (i.e. sets of instances testing a common skill). Inspecting accuracy over these slices yields novel insights on model trade-offs: e.g., compared to GPT-4o and Claude 3.5 Sonnet, on average, Gemini 1.5 Pro is $18\%$ more accurate in "computing molar mass", but $19\%$ less accurate in "applying constitutional law", despite the overall accuracies of the three models differing by a mere $0.4\%$. Furthermore, we demonstrate the practical utility of our approach by showing that insights derived from skill slice analysis can generalize to held-out instances: when routing each instance to the model strongest on the relevant skills, we see a $3\%$ accuracy improvement over our $12$ dataset corpus. Our skill-slices and framework open a new avenue in model evaluation, leveraging skill-specific analyses to unlock a more granular and actionable understanding of model capabilities.

==> contents/2_method_new.tex <==
% \newpage
\section{Constructing skill-slices using Model-Generated Rationales}
% \section{Extracting and Aggregating Localized Skills from Rationales}
\label{sec:method}
% We now detail our method for inferring relevant skills for each evaluation instance and aggregating skill annotations across datasets to form \emph{skill-slices} (i.e. a set of instances that share a relevant skill). We utilize \emph{rationales}, or step-by-step solutions, generated by a strong model (GPT-4o) to facilitate the extraction of relevant skills, as explained in \S~\ref{subsec:skill-extraction}. However, as evaluation instances are challenging by design and generating relevant skills requires a significant level of meta-reasoning, it is important to asses the quality of produced skills.
% % generating relevant skills requires a level of meta-reasoning that models may not possess, especially since evaluation instances are challenging by design. 
% Thus, in \S~\ref{subsec:verifiers}, we additionally present a multifaceted automatic approach to validating the relevance of extracted skills, which we confirm aligns well with human judgements. 

We now detail our method for inferring relevant skills for each evaluation instance. We utilize \emph{rationales}, or step-by-step solutions, generated by a strong model (GPT-4o) to facilitate the extraction of relevant skills, as explained in \S~\ref{subsec:skill-extraction}. However, as evaluation instances are challenging by design and generating relevant skills requires a significant level of meta-reasoning, it is important to asses the quality of produced skills. Thus, in \S~\ref{subsec:verifiers}, we present an automatic approach to verify the relevance of extracted skills, which we confirm aligns well with human judgements.
Applying this verification, we find that skill annotations are indeed reliable. 
Then, in \S~\ref{subsec:slices}, we aggregate skill annotations across datasets to form \emph{skill-slices} (i.e. a set of instances that share a relevant skill), with which we will compare models in \S~\ref{sec:findings}. 

\subsection{Skill Extraction via Rationale Parsing}
\label{subsec:skill-extraction}
Given an evaluation instance, we prompt GPT-4o to generate a detailed rationale (i.e. step-by-step solution), where each step only involves the use of a single skill; figure \ref{fig:methods_diagrams} presents an example. We additionally instruct the model to, after each step, list the applied skill with \emph{multiple} names of \emph{cascading granularity}. For example, the skill `treble clef recognition' is prepended with `perception, visual recognition, symbol identification'\footnote{If some of these skills are unfamiliar to you, you're not alone! Many benchmarks today ask questions that are challenging to anyone without expertise in the relevant domain. This precisely motivates relying on stronger models to help us make sense of these benchmarks, as manual inspection has increasingly limited utility.}. Listing multiple names of different granularity per skill is a simple way to increase the number of slices an evaluation instance falls into, leading to a greater quantity and diversity of skill-slices. Further, each granularity has unique and complementary advantages: fine-grained skills are more specific, while coarse-grained skills lead to slices with a larger number of samples, making an accuracy estimate over such slices more reliable. Also, in order to standardize the response structure, we include an in-context example in our prompt, which enables simple parsing of rationales to extract skills. See Appendix \ref{app-sec:prompt} for complete details.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/methods_diagram.png}
    \caption{\textbf{(left)} Sample GPT-4o generated rationale: each skill is listed under multiple names of \emph{cascaded granularity}, and localized to a specific step and concluding claim. \textbf{(right)} Annotated skills can be verified independently with a second model or human. We include randomly sampled negative skills and multiple verifiers to assure the quality of the verification, as detailed in \ref{subsec:verifiers}.}
    \label{fig:methods_diagrams}
\end{figure}

\looseness=-1
Note that other methods could possibly be used to annotate relevant skills, like directly prompting GPT-4o to list them. We prioritized maximizing the total count and size of resultant skill-slices, so to create more dimensions of varied granularity with which we can compare model performance. In comparing the skills per instance obtained by direct prompting vs. our rationale parsing, we indeed find that rationale parsing results in a higher average count and diversity in grain (Appendix \ref{app-sec:prompt-ablation}). 

\begin{figure}
    \centering
    \begin{minipage}{0.4\linewidth}
    \includegraphics[width=\linewidth]{figures/skill_verification_confmats_all.jpg}
    \end{minipage}
    \begin{minipage}{0.5\linewidth}
    \includegraphics[width=\linewidth]{figures/verification_cc_vs_not.png}
    \end{minipage}
    \caption{(\textbf{left}) Post-hoc verification shows GPT-4o-annotated skills are relevant, and that automatic verifiers are reliable, as they admit low rates of false positives (marking a randomly sampled negative skill as relevant). (\textbf{right}) Rate that GPT-4o-annotated skills are marked as relevant, separated by if GPT-4o correctly answered the underlying evaluation instance (blue) or not (orange). Empirically, annotated skills have high relevancy rates \emph{even} when the annotator incorrectly answers the question.}
    \label{fig:validation}
\end{figure}

\subsection{Automated Validation of Skill Relevance}
\label{subsec:verifiers}
\looseness=-1
As evaluation instances are challenging by design, leading to errors by even the strong models used to generate rationales, we must first verify the reliability of automatic skill annotations before using them to gain evaluation insight. Our skill annotations are finer-grained than existing manual annotations, restricting our ability to compare to established ground truth. Further, while automated skill annotations may be accurate for one set of instances, they may not be for another set of instances that are harder or from a different domain.

% Thus, a scalable manner to verify the reliability of automatic skill annotations is required to trust the insights gained by inspecting accuracy over skill-slices.

\looseness=-1
Thus, we propose two automated methods to directly and scalably validate the relevancy of listed skills: \emph{post-hoc verification} and \emph{inter-(skill)annotator agreement}. The latter checks the overlap in skills listed for the same instance by two different annotators. Here, we focus on the former and defer full details of both approaches to Appendix \ref{app-sec:validation}. Post-hoc verification consists of a second `verifier' model which inspects an evaluation instance with a list of skills and marks whether each skill is relevant or not.
We form the list of skills by combining the skills for the instance with an equally sized list of \emph{negative} skills, randomly sampled as follows: with $S$ denoting all skills from our corpus, negative skills for an instance $x$ with skills $S_x$ are drawn from $\{s \in S \mid \max_{s_i \in S_x}\text{sim}(s, s_i) \leq \tau\}$. Here, `sim' is the similarity of two skills, computed via the cosine similarity of text embeddings from a frozen text embedder. The threshold $\tau$ is selected based on the text embedder so that no negative skill is equivalent up to paraphrasing to an annotated skill for the instance. We include negative skills as quality controls to ensure that the verifier model does not simply mark all skills as relevant.
% Like attention checks for human annotators \citep{mturk_quality_assurance}, the randomly sampled negative skills serve as quality controls to ensure that the verifier model does not simply mark all skills as relevant.
% \varun{bad analogy i think? llm's don't get tired. in fact, prior work has shown that these models get distracted by irrelevant context (\url{https://arxiv.org/abs/2302.00093})} \mazda{while attn checks for humans are because they may get tired, in general they are just quality controls, which we also need in our case.}

\looseness=-1
Figure \ref{fig:validation} shows the results of post-hoc verification of skills for $100$ skills per dataset averaged over three verifier models (\ClaudeSonnet, \GeminiPro, GPT-4v\footnote{GPT-4v denotes \GPTFourTurboApril, and GPT-4o denotes \GPTFourO throughout our paper.}). We observe $94.1\%$ of skills annotated by GPT-4o are verified as relevant. A smaller scale human validation of $640$ total skills results in $95.7\%$ relevancy rate, as well $92.8\%$ agreement with automatic verifiers, indicating that post-hoc verification is a reliable automated metric for assessing skill relevancy. 
% fel :These findings indicate that post-hoc verification is a reliable automated metric for assessing skill relevancy.
% \vibhav{Filling placeholders X, Y, Z.}
The right panel shows that the relevancy rate is roughly equivalent, \emph{regardless of if the annotator correctly answers the underlying evaluation instance}; crucially, this enables using automated skill annotations on instances that are interesting to evaluate on (i.e. hard enough to stump some models). 
%Further, the results suggests that models can describe how to solve a problem even when they cannot apply the skills they articulate are relevant. 
Thus, while rationales may at times be partially incorrect\footnote{In fact, there's an error in the rationale in Figure \ref{fig:methods_diagrams}: the notes are $B\flat$ \& $C$. However, the skills are accurate.}, they can still be leveraged to shed insight on \emph{data} at scale.

\subsection{Curating \emph{skill-slices} Across Benchmarks}

\looseness=-1
\textbf{Remark: \textit{Skills cut across benchmarks.}} We tag relevant skills for $46k$ evaluation instances from 12 benchmarks that are popular (i.e. commonly featured in evaluations for recent model releases) and unsaturated (SOTA under $90\%$ accuracy), resulting in $690k$ total skills ($128k$ unique) over $202k$ distinct rationale steps. Since skills are re-used, many skill-slices of non-trivial size are formed when including instances across benchmarks. Namely, $278$ skills have at least $100$ unique instances each. This number rises to $332$ after de-duplicating via a tight clustering\footnote{We employ a high minimum cosine similarity threshold of $0.95$ per cluster to de-duplicate skills listed under slightly different names; e.g., `trigonometry' and `trigonometric calculation' have a similarity of $0.95$.} on the text embeddings of the skills. This cross-benchmark analysis also enables us to analyze skills that perhaps may be in the long tail for one benchmark, but get resurfaced when many different benchmarks are joined together. 
% We will release all code to enable the community to expand on our annotations, adding new benchmarks as desired.

Effectively, our skill-slices are like new `splits' of existing evaluation instances based on the model ability they test. Splits like these are already a feature of some benchmarks \citep{mmtbench, liu2024mmbench, eureka}, though in those cases, they are the result of manual curation or creation of instances. We hope our method can serve as a cost-effective alternative, so that the more expensive manual work can be reserved for abilities our method flags as potentially deficient. 




% \textbf{Caveats.} \mazda{maybe we can move this to a limitations (appendix?) section. All I want to say is (i) we don't claim rationales to be correct or faithful (noted above), and that (ii) skill annotations may not be \emph{complete} (which explains the higher false positive rate of 9\%), but we have reasonable inter-annotator agreement and some skills are better than none. In general, the high rates of agreement both across annotators and verifiers supports the claim that the skills we extract in this stage are a property of the data (maybe this point is obvious?). I dont want ppl to get confused here thinking that I am talking about extracting the skills/abilities of GPT-4o... maybe I need to emphasize this at the start of the section.} \vibhav{Good last point that the reviewers should not get confused. Apart from emphasis, we could also highlight skill discovery by other models as well.}

% \vibhav{Are we giving a summary of the dataset and annotated skills here? For example, which datasets were considered? Which ones are for LLM and for LMM? How instances were considered? How many final list of skills did we get?}

% Lastly, we note that our verification shows high relevance of the annotated skills, but it does not measure the completeness. That is, it is possible other skills may be relevant to a given evaluation instance that our procedure does not extract; e.g., if a two solutions engaging slightl different sets of skills can be taken, and our annotator only outlines one such solution. Some mechanisms to improve completeness include 

% sanity checks to corroborate the insights obtained from our skill-slice analysis

% \subsection{Sanity Checks via Skill Localization}
% \mazda{I think we move this to after section 3, so that we get to the cool findings faster and so that the probing explanations appear right next to the probing results. Also, I don't want to cast doubt on skill-wise accuracies so early (since we discuss how they can admit false positives; note that this is a problem for any single annotation, not just us). Maybe we can include the inter-annotator agreement here bar plots after all.}

% \looseness=-1
% Rational parsing also allows for each skill to be \emph{localized} to a specific step, as well as the resulting claim, which we instruct models to include. For example (fig. \ref{fig:methods_diagrams}c), the resultant claim to a step where the skill \emph{musical note identification} is applied would be \emph{The notes are B and E}. A claim can then be reframed as a question (e.g. \emph{what are the notes?}) probing a single skill, unlike the original question that often requires numerous skills and steps, any one of which could cause an incorrect answer. Then, \emph{consistency} over multiple responses to a probing question can shed insight on if a model is proficient at the probed skill: if a model contradicts itself, it must have been wrong at least once.

% Importantly, this offers a \emph{complementary} signal to the one obtained by inspecting model accuracy over a skill-slice. Namely, since evaluation instances typically engage multiple skills, low accuracy over one skill-slice may be due to a deficiency on another highly co-occurring skill. However, if a model is proficient in a skill, it will always answer consistently to probing questions. Conversely, while a true skill deficiency for a model (i.e. causing it to fail anytime the skill is relevant) will always result in low accuracy over the skill-slice, the model could have consistency on probing questions for the deficient skill by always answering incorrectly in the same way. 

% We leverage consistency over probe questions as a sanity check on skill-slice accuracies given a model. While these techniques approach measuring skill-wise performance from opposite directions, we find that their results corroborate one another: as we'll show in section \ref{sec:consistency-results}, models indeed have higher rates of inconsistency on skills with low accuracy over their slices. %Further, using these two techniques in sequence can refine evaluation output, so to obtain true skill deficiencies. 

% \mazda{this should be at the start of the section} Recall that our skill extraction aims to uncover the skills each evaluation instance tests, \emph{not} directly discern what skills a model possesses. To proxy the proficiency of any model for a given skill, we can inspect accuracy over the corresponding skill \emph{slice} (set of instances where the skill is marked as relevant).



% \varun{may want to reiterate the higher level objective once more}

% We now detail the creation of the \skillset, our corpus of $60k$ curated evaluation instances with skills automatically annotated and localized to specific claims \varun{what is a claim?}. Broadly, we selected benchmarks featured in the evaluations for recently released frontier models, with an emphasis on multimodal tasks and benchmarks where models were not yet saturated. \varun{before you detail the procedure, you want to explain "why" you want to do this particular set of steps: what are the challenges you wish to overcome?} Then, we crafted a prompt for GPT-4o to generate a rationale with skills listed per step, given any instance. Finally, after parsing skills from these rationales, we aggregate skills across benchmarks and deduplicate them via a tight clustering. 

% Concretely, [write above in math notation? only if it would improve clarity]

% Figure \ref{sample_rationale} summarizes our framework, from instance-wise skill annotation to cross-benchmark skill clustering. Focusing on skill annotation, we now delve into two specific choices made in crafting our prompt, towards achieving (a) easy parsing of the skills along with their associated claims (b) maximal coverage of relevant skills (c) breadth in grain of skills listed. \mazda{todo: say choice of prompt is not critical -- we choose one that works for us, but others can modify if they e.g. don't need probing qs or coarse skills}

% First, instead of directly prompting GPT-4o to list relevant skills given an evaluation instance, we instruct the model to generate a \emph{detailed rationale} (i.e. step-by-step solution), where each step only utilizes a single skill. 
% %We elect rationale parsing so to maximize the number and type of skills listed. 
% Since skill annotations relate to \emph{how} an instance is solved, we conjecture that rationale parsing may capture more skills than prompting a model to list skills directly. Further, models have been observed to be adept at generating such rationales \citep{orca2}, and in general benefit from thinking step by step \citep{think_step_by_step}. Lastly, and most distinct from direct prompting, rationale parsing enables \emph{localization} of skills to specific claims. We utilize these claims to form probing questions that isolate a skill of interest, toward refinement (and validation) of purported skill deficiencies by way of consistency checks (detailed in section \ref{sec:consistency}). 

% Next, for each skill, we request GPT-4o to provide \emph{multiple names with cascaded granularity}. For example, `treble clef recognition' is prepended with `perception, visual recognition, symbol identification'. Listing multiple names of different grains per skill is a simple way to increase the number of slices an evaluation instance falls into, which in turn leads to the creation of a greater quantity and diversity of skill-slices. Further, including coarse-grained names leads to skill-slices with a larger number of samples, making an accuracy estimate over such a slice more reliable.


% \looseness=-1
% \textbf{\textit{Remark: Skills cut across benchmarks.}} We tag relevant skills for $46k$ evaluation instances from over a popular dozen benchmarks, resulting in $690k$ total skills ($128k$ unique) over $202k$ distinct rationale steps. Since skills are re-used, many skill-slices of non-trivial size are formed when including instances across benchmarks. Namely, $322$ skills are tagged for at least $75$ unique instances. This number rises to $441$ after deduplicating via a tight clustering\footnote{We employ a high minimum cosine similarity threshold of $0.95$ per cluster to deduplicate skills listed under two slightly different names; e.g., `trigonometry' and `trigonometric calculation' have a similarity of $0.95$.} on the text embeddings of the skills.  

% \mazda{Worth making explicit mention that we do not require rationales to be faithful. Also that our annotated skills cut across benchmarks in a way that original meta-annotations provided by benchmark creators do not. Also that our code will be public and it is extremely easy to get skill annotations for any new benchmark; we should comment how long (and how expensive) skill annotation is though.}

% \textbf{Remark: Our framework is flexible and general.} We put forward skill annotations for over a dozen benchmarks as a v0, and emphasize that incorporating new benchmarks is easy: we release all code for prompting, parsing, and deduplicating skills, as well as code for automated validation of annotated skills, using methods we describe in section \ref{sec:validation}. The longest step is generating rationales, which GPT-4o can do X instances per minute at a cost of Y on average. 

% We need to explicitly differentiate a `skill' from an attribute of the input. Main points: a \textit{skill} is a property of the solution, not just the input or the output. Thus, to uncover skills, we prompt a strong model to provide a detailed rationale, enumerating the skills associated with each step of the solution. 

% Add nomenclature/glossary of key terms: Rationale, skills, tasks, benchmark, evaluation

% An evaluation benchmark $\mathcal{B}$ consists of a set of instances $q$, where each instance contains some input to a model $q_{in}$ and a metric to measure the alignment of the consequent model output to a desired outcome (typically provided as a ground truth). For example 

% KEY CLAIMS: 
% \begin{enumerate}
%     \item GPT-4o can list skills relevant to instances in popular benchmarks, even when it cannot solve those instances.
%     \item Our prompting technique can increase the quantity (via rationale) and diversity in grain (via cascaded naming) of skills listed. 
% \end{enumerate}

% \begin{enumerate}
%     \item Skill annotation (f: Problem → List of localized skills).\\
%     Challenges: precision and coverage of annotated skills
%     \item Skill dedup/merge/clustering
%     \item Probe generation: claim retrieval, prompting
%     \item Consistency check
% \end{enumerate}

% \opportunity

% Define a \textbf{total} skill deficiencies as a skill $s$ for model $f$ such that any instance that requires skills $s$ is answered incorrectly. If a sufficient number of instances that require $s$ exist in the corpus, our two stage pipeline identifies these skill deficiencies perfectly, because stage one has perfect recall (while admitting false positives) and stage 2 has perfect precision (while admitting false negatives).  

% \begin{remark} 
% Two-stage pipeline identifies \textbf{total} skill deficiencies with perfect precision.
% \end{remark}



==> contents/old_intro.tex <==
\section{Introduction}

% \varun{i like your intro flow!}
% \vidhisha{+1 like the motivation and structure, the experiments part of intro is a bit dense in info but we can work on organizing it :)}

Recent years have seen benchmarks evolve to keep up with ever-advancing models. While classical benchmarks tested specific capabilities, like recognizing digits \citep{lecun1998mnist} or classifying sentiment \citep{bowman2015snli}, modern benchmarks measure proficiency in numerous capabilities simultaneously, drawing questions of increasing difficulty from more diverse domains \citep{mialon2024gaia, yue2023mmmu, wang2024mmluprorobustchallengingmultitask}. As the questions we test models on have grown more complex, aggregate performance measures provide less understanding about model proficiency in specific abilites. 
%, limiting the utility of evaluations to understand trade-offs between models. 
For example, as shown in Figure \ref{fig:teaser}, we find that over a dozen benchmarks, GPT-4o, \GeminiPro, and \ClaudeSonnet \citep{openai2024gpt4o, geminiteam2024gemini15unlockingmultimodal, anthropic2024claude35sonnet} achieve overall accuracies within $0.4\%$ of one another, leaving an open question: Are these models all the same, or are valuable insights being averaged away?

\looseness=-1
Manual annotations of categories across instances (e.g. \cite{mmtbench} and \cite{liu2024mmbench} include `ability' tags) enable going beyond accuracy, but at a cost for benchmark creators that rises with the number and difficulty of test questions. This results in few (if any) and non-standardized annotations, restricting cross-benchmark aggregation, even though many benchmarks have large overlap in the skills they test \citep{miao-etal-2020-diverse, cobbe2021gsm8k}. Prior works show promise in automatically grouping inputs by attributes to extract image classification failure modes (e.g. `fails on \emph{white} foxes') \citep{eyuboglu2022domino, rezaei2024prime}, but these methods fail to produce deeper insights on the underlying competencies that models use across contexts (e.g. `fails on \emph{counting}').

To this end, we propose a method to automatically discover \emph{skills} related to any evaluation instance, toward a finer-grained understanding of model capabilities from existing benchmarks. We consider skills as latent features pertaining to ``how'' a model must operate -- the steps involved in solving a given task -- whereas a general attribute relates to ``what'' is being addressed -- the observable characteristics of the instance. Moreover, the relevant skills for an instance may not be readily apparent through superficial examination, often only revealing themselves upon inspection of the solution. 
This complexity highlights the challenge of automatically inferring relevant skills and underscores the need to develop new approaches for their effective identification.
% If and how relevant skills can be inferred automatically is an open question that requires new approaches that we investigate in this work


% As such, relevant skills may not be clear at first glance of an instance, only becoming more apparent when considering its solution. If and how relevant skills can be inferred automatically is an open question that requires new approaches that we investigate in this work.

% While attribute level analysis is useful for informing methods that extend the generalization of models in terms of content (e.g. addressing OOD cases like white foxes), skill level analysis is useful for informing methods that extend the generalization of models in terms of functionality and capabilities (e.g. counting, spatial reasoning).


% In pursuit of a scalable alternative to manual annotation, we investigate if models can shed insight on the benchmarks we have created for them. Prior works shows promise in automatically grouping data for the image classification setting: \cite{eyuboglu2022domino} and \cite{rezaei2024prime} use image encoders and taggers respectively to find failure modes based on shared surface-level attributes (e.g. `fails on \emph{white} foxes'). In our work, we propose to infer a deeper property that exists for \emph{any} evaluation instance: the \emph{skills} relevant to solving the instance. 

% Attribute level analysis is useful for informing methods that extend the generalization of models in terms of content and address OOD problems(e.g. white foxes). Skill level analysis is useful for informing methods that extend the generalization of models in terms of functionality and capabilities (e.g. counting, spatial reasoning). While both types of analysis are useful, the former is more apt for analyzing and improving single capabilities (e.g. object recognition), while the latter is needed for analyzing more general models for whom the expectations expand a myriad of skills and capabilities.

% \looseness=-1
% A skill is distinct from a general attribute in that it pertains to what a model must \emph{do}. Indeed, two instances sharing surface-level attributes can require disparate skills for a model to solve them. Thus, skill annotations offer complementary signal to attributes that is useful when analyzing general-purpose models beyond a single capability, as it may more directly capture underlying model abilities that are re-used in many settings. Further, relevant skills may not be clear at first glance of an instance, only becoming more apparent when considering its solution. If and how relevant skills can be inferred automatically is an open question that requires new approaches that we investigate in this work.
% as i said, i think you define skill by contradiction, i would propose a clear definition as it's the core of the paper, here is my proposition: 
% A skill is distinguished from a general attribute in that it pertains to ``how'' a model must operate -- the reasoning processes, methodologies, or strategies it employs to solve a task -- whereas an attribute relates to ``what'' is being addressed -- the observable characteristics or outcomes of the instance. Indeed, two instances may share identical attributes yet require entirely disparate skills for a model to solve them. Thus, skill annotations offer complementary insights to attributes by more directly capturing the underlying competencies that models use across diverse contexts. Moreover, the relevant skills necessary to solve an instance may not be immediately apparent upon superficial examination and often become evident only through an analysis of the solution process. This underscores the complexity of automatically inferring pertinent skills and necessitates the development of novel approaches to identify them effectively.


% \vidhisha{why do we need a deeper skill aspect? we should motivate with some shortcomings of attribute based insights} \mazda{explain more of what is a skill}
% \vidhisha{yes this seems more than we need. Just one line about why skills should be sufficient. Suggestion: In our work, we propose to infer a deeper property that exists for \emph{any} evaluation instance: the \emph{skills} relevant to solving the instance. Skills, differing from surface level attributes enable more latent and fine-grained insights into the problem solving capabilities of our models.}

%%% Prev paragraph with comments
% Manual annotations of broader categories across instances (e.g. \cite{mmtbench} and \cite{liu2024mmbench} include `ability' tags \varun{add something to say that this is hard?}) enable going beyond accuracy, though at a cost that rises with the number and difficulty of test questions \varun{i would move the example here}. This cost falls on the shoulders of benchmark creators, resulting in few (if any) and non-standardized annotations, restricting cross-benchmark aggregation. \varun{downside for not being able to aggregate across benchmarks? you can state that there are numerous benchmarks evaluating the same thing e.g., GSM8K, MATH etc, so it would be cool to homogenize?} In pursuit of a scalable alternative, we investigate if models can shed insight on the benchmarks we have created for them. Prior works show that grouping data based outputs of auxiliary models like image encoders \citep{eyuboglu2022domino} or taggers \citep{rezaei2024prime} allows for extracting interpretable failure modes \varun{do you want to say failures? or insights?} based on surface level attributes (e.g. `fails on white foxes'), indicating promise in this direction, though in a simple setting. In our work, we propose to infer a deeper quality \varun{is quality the right word?} that exists for \emph{any} evaluation instance: the \emph{skills} relevant to solving the instance. \vidhisha{why do we need a deeper skill aspect? we should motivate with some shortcomings of attribute based insights} \mazda{explain more of what is a skill}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/tmp_teaser.png}
    \caption{Work in progress teaser. May add simple e2e schema above.}
    \label{fig:teaser}
\end{figure}

\looseness=-1
We propose to harness the \emph{rationale}-generating ability of strong models to infer skills, as rationales (i.e. explained solutions) elucidate the steps involved in performing a task. Eliciting rationales has had many benefits, like improved accuracy \citep{wei2022chain, kojima}, explanations \citep{Singh2024RethinkingII, xai_rationales}, and distillation \citep{orca2, hsieh2023distilling}; in our work, we leverage rationales  

% While some question rationale faithfulness to (and existence of) model `reasoning' \citep{madsen-etal-2024-self, huang-chang-2023-towards}, we side-step these concerns by using rationales not to directly analyze the rationale-generating model, but instead to annotate \emph{data}, on which \emph{any} model can be evaluated. 


%%% Prev paragraph w comments
% To do so, we harness the ability of strong models to generate \emph{rationales}. Eliciting rationales has had many benefits, like improved accuracy \citep{wei2022chain, kojima}, explanations \citep{Singh2024RethinkingII, xai_rationales}, and distillation \citep{orca2, hsieh2023distilling}. While some question rationale faithfulness to (and the existence of) inherent model `reasoning'\citep{wang2023pinto, huang-chang-2023-towards}, we side-step these concerns by using rationales not to directly probe \varun{maybe do not use probe? maybe "directly understand"?} the rationale-generating model, but instead to annotate \emph{data}, on which \emph{any} model can be evaluated. \vidhisha{I'm not sure we need to introduce the confusion on faithfulness here - plus it doesn't contribute to your work anyway.}

% \looseness=-1
Specifically, given an evaluation instance, we instruct a strong model (e.g. GPT-4o) to generate a detailed rationale consisting of the steps needed to solve the problem, along with the skill applied in each step. We then parse skills per instance for numerous benchmarks and aggregate instances along skill \emph{slices}, i.e. subsets of instances drawn from multiple benchmarks that all involve a specific skill, enabling measurement of model proficiency for that skill. After applying our technique to over $45k$ instances from a dozen popular modern benchmarks (primarily multimodal), we find \emph{hundreds} of skills with slice sizes of $\geq100$, which we will release, along with all rationales, to the community. 

% articulating the skill used per step \varun{the last bit of the sentence is dense; you want to explain that the rationale explains how the problem is solved in multiple-steps, and you want a skill associated with each step?} \vidhisha{+1}. Our prompt is effective \varun{effective how?} for multiple rationale-generating models (not just GPT-4o), and we confirm that the skills listed are indeed relevant -- notably, even on instances where GPT-4o answers incorrectly -- via human and automated validation. \vidhisha{experiment details are very vague here. i think we should separate the methodology (eliciting skills) and experiments (validation+insights)} 

% \looseness=-1
Additionally, as models are known to hallucinate \cite{huang2023surveyhallucinationlargelanguage} and evaluation instances are challenging by design, we devise an automatic verification protocol to assess if rationale-parsed skills are relevant. Interestingly, we observe the skills to indeed be relevant even for instances that the rationale-generating model answers incorrectly. Having validated the fidelity of our skill slices, we then demonstrate their utility to understand trade-offs of commercial models from OpenAI, Google, and Anthropic, while only needing black-box access. Namely, skill slices reveal \emph{unique strengths and weaknesses} of each model, as well as \emph{newfound abilities from one model release to the next}.  

% After parsing skills from rationales generated for a dozen popular modern benchmarks (primarily multimodal), we aggregate skills across $45k$ (evaluation) instances  to enable the indexing of hundreds of \emph{skill slices} (i.e., sets of instances drawn from multiple benchmarks that all involve a single skill). With skill slices, we can more deeply understand trade-offs across models \varun{models' performance?}, while only needing black-box access. We demonstrate this by presenting new findings on commercial models from OpenAI, Google, and Anthropic . \varun{move this last sentence earlier?} We note that we will release all skill annotations, to enable richer evaluation insights for the whole community. 
%%% Prev paragraph with comments
% Specifically, given an evaluation instance, we instruct a strong model (e.g. GPT-4o) to generate a detailed rationale, articulating the skill used per step \varun{the last bit of the sentence is dense; you want to explain that the rationale explains how the problem is solved in multiple-steps, and you want a skill associated with each step?} \vidhisha{+1}. 
% Our prompt is effective \varun{effective how?} for multiple rationale-generating models (not just GPT-4o), and we confirm that the skills listed are indeed relevant -- notably, even on instances where GPT-4o answers incorrectly -- via human and automated validation. \vidhisha{experiment details are very vague here. i think we should separate the methodology (eliciting skills) and experiments (validation+insights)} \mazda{expand on challegnes} After parsing skills from rationales generated for a dozen popular modern benchmarks (primarily multimodal), we aggregate skills across $45k$ (evaluation) instances  to enable the indexing of hundreds of \emph{skill slices} (i.e., sets of instances drawn from multiple benchmarks that all involve a single skill). With skill slices, we can more deeply understand trade-offs across models \varun{models' performance?}, while only needing black-box access. We demonstrate this by presenting new findings on commercial models from OpenAI, Google, and Anthropic . \varun{move this last sentence earlier?} We note that we will release all skill annotations, to enable richer evaluation insights for the whole community. 

\looseness=-1
Figure \ref{fig:teaser} illustrates a snapshot of the practical insights our method enables. Despite roughly equal average accuracy across our corpus for the three models, we discover skills for each of GPT-4o, \GeminiPro, and \ClaudeSonnet where accuracy far exceeds that of its counterparts, with gaps as large as $20\%$. For example, we find \GeminiPro to be much stronger in mathematical skills, like \emph{setting up equations}, while falling far behind for legal skills like \emph{applying constitutional law}. When comparing releases from each family, we find that while \GeminiPro did not improve over v1.0 on \emph{understanding legal procedures}, OpenAI and Claude models improved substantially, with \ClaudeSonnet leaping nearly $50\%$ over \ClaudeOpus (far greater than the $8.7\%$ average improvement observed over all instances). We also present a proof of concept for how skill-wise accuracies can enable more calculated model selection: when routing each instance to the model with the best accuracies on the relevant skills, overall accuracy over a dozen benchmarks improves by $3\%$ absolute, including gains of $4$ to $7\%$ on MMLU Pro \citep{wang2024mmluprorobustchallengingmultitask}. The success of this simple, training-free routing approach shows that that insights from skill-slice analysis can generalize to new settings.

%%% Previous paragrpah w/ comments
% An example of such insights is {\em revealing newfound abilities from one model release to the next}: while Claude-Sonnet improves $8.7\%$ on average over Claude-Opus, legal skills see far greater improvements, leaping nearly $50\%$. Further, as shown in figure \ref{fig:teaser}, we discover skills for each of GPT-4o, Gemini-1.5-pro, and Claude-Sonnet 3.5 where accuracy far exceeds that of its counterparts, with gaps as large as $20\%$, despite roughly equal average accuracy across our corpus for the three models. For example, we find Gemini to be much stronger in mathematical skills, while GPT-4o excels in visual skills related to color and locating objects. We also present a proof of concept for how skill-wise accuracies can enable more calculated model selection: when routing instances \varun{want to explain what routing means in this context?} to the model with best accuracies on the relevant skills, overall accuracy over a dozen benchmarks improves by $3\%$ absolute, including gains of $4$ to $7\%$ on MMLU Pro \citep{wang2024mmluprorobustchallengingmultitask}. The success of this simple, training-free routing approach offers validating signal that insights from skill-slice analysis can generalize to new settings. \vidhisha{i think this paragraph could use some structure - first listing broadly the set of ways you use skills and then insigts from each?}

\looseness=-1
Going deeper than skill slices, we show how rationales enable assessing the proficiency of models to apply skills \emph{in isolation}. Specifically, in rationales, each skill is \emph{localized} to a specific step and concluding claim. By reframing the claim, we generate probing questions that directly target a specific skill and can be used to devise a complementary metric of skill proficiency. Importantly, we find this metric to corroborate skill slice accuracies. Thus, while instances within skill slices may still involve multiple skills simultaneously, a second analysis enabled through our framework offers evidence that slice accuracies can proxy proficiency for the articulated skill alone.  

%%% old paragraph
% Rationales also enable digging deeper than skill slices, thanks to skill \emph{localization}. That is, for any skill, we can surface specific steps where the skill was applied, from which \emph{probing questions} can be generated that isolate the skill more so than the original evaluation instance. \mazda{split this sentence} When we compute the rate that models contradict themselves over multiple answers to the same probing questions, we find double and triple rates of inconsistency for skills with low slice accuracy than average or high accuracy respectively, corroborating the findings of our skill-slice analysis. 

% \looseness=-1
% Lastly, we show how custom skill slices can be retrieved from our corpus via open-vocabulary query. We find that searching over embeddings of skill annotations is far more precise than searching over embeddings of the evaluation instance directly. In addition to creating a flexible way to engage with the skill annotations we'll release, these results show that the skills an instance tests is a more latent property than the surface-level attributes prior auto-error-analysis works group instances by. Thus, our method offers novel, complementary insight to prior works on image classifier failure mode extraction, while also being far more general. \mazda{Honestly maybe we can just omit this in the intro... feels out of place}

% In summary, we present an automated manner to enrich black-box evaluations, leveraging the rationale-generation abilities of today's strong models to gain valuable insight on (i.e. the skills tested by) arbitrary evaluation instances. Analysis on skill slices formed by aggregating instances across benchmarks reveal novel findings on the trade-offs between leading commercial models. Results on skill-based routing suggest that skill-slice accuracies are predictive of performance on held-out instances and potentially useful in improving overall performance. Finally, probing questions help isolate individual skills, offering complementary and corroborating signal to our insights from skill-slices. As evaluation instances grow harder to keep up with advancing models, making sense of performance on these instances will become more challenging too. We hope our framework can help the community gain deeper understanding from the evaluations of today, and tomorrow.%, towards a deeper understanding of model abilities. 

% \mazda{more concise; perhaps bullet points of key contributions (method, released skill-slices, key insights)}

% \vidhisha{More detailed comments: I like the motivation of your work, i would just separate our the two problems you're addressing - insights and scale - to be more explicitly called out. In the methodology and experiment details, there are a lot of details which is amazing and what we want but a bit mixed together, so clearly structuring it as 1) proposed idea, 2) description of methodology, 3) validating quality 4) what experiments you ran 5) main insights and 6) reiterating benefits/contributions. This helps follow the paper also!}

% \mazda{more discussion on `why skills'. Two solutions can have diff failure causes; attr may not catch this}

\begin{comment}
0. why is inferring skills non trivial? response: previous approaches that based on direct embedding of the instance may offer complementary characterization of the instance, but this is not precise? for example: .... 
0a. additionally, our approach is black-box, which has its own pros
1. why should i trust skills? response: human validation on a small set + another strong model validates, and it's unlikely that two models will come to the same incorrect conclusion
2. why is the granularity of skills the right one? response: previous approaches have no notion of granularity. they have one option; this may suck because it may inhibit aggregation across multiple datasets; it may also suck because it's not fine enough to give you a deeper understanding of specific behaviors. our approach allows for this flexibility. however, if we go down the "fine grain" route, we will have many skills per instance and it will be hard to isolate the effects of any one skill on the behavior of the model on that sample; to this end - we come up with a mechanism to generate probing questions...
\end{comment}
